A Roadmap for Software Testing in Open Collaborative Development Environments

Amidst the ever-expanding digital sphere, the evolution of the Internet has not only fostered an atmosphere of information transparency and sharing but has also sparked a revolution in software development practices. The distributed nature of open collaborative development, along with its diverse contributors and rapid iterations, presents new challenges for ensuring software quality. This paper offers a comprehensive review and analysis of recent advancements in software quality assurance within open collaborative development environments. Our examination covers various aspects, including process management, personnel dynamics, and technological advancements, providing valuable insights into effective approaches for maintaining software quality in such collaborative settings. Furthermore, we delve into the challenges and opportunities arising from emerging technologies such as LLMs and the AI model-centric development paradigm. By addressing these topics, our study contributes to a deeper understanding of software quality assurance in open collaborative environments and lays the groundwork for future exploration and innovation.

==> section/response.tex <==
\section{Response to Reviewers}

\subsection*{Response to Editor}

We have carefully reviewed the comments and suggestions provided by the reviewers. 
Following this, we offered clarifications on the points highlighted by the reviewers and revised our manuscript accordingly. 

\subsection{Response to Reviewer \#1}

\review{\textbf{Review:} The present submission consists of remarkable revision of a previously submitted paper, that analyzes the most prominent literature contributions about software testing based on machine learning. The presentation of relevant literature brings the discussion to open problems and promising research directions in this research field. }

\review{\textbf{Review:} In my previous review I raised a major concern about the approach used to collect related work, and I asked authors to a adopt a more systematic and structured methodology to ensure survey completeness. However, as pointed out in the response letter, such structured approaches might be difficult to apply to a such wide topic. It might be appropriately applied separately to each single subsection of this submission, but not to all the sections at once. So, to keep a wide overview angle in presenting the paper topic, a more informal mapping approach should be kept, mainly focusing only on papers published in top venues.}

\review{\textbf{Review:} I agree with the authors and now I share their vision that the methodology previously suggested by me was not the most appropriate for this submission, so I'm quite happy with authors answer. Nonetheless, I would still recommend to mention this "informal" methodology in the paper, and report the informal process used to assemble relevant work (similarly to what authors answer in the letter) based on authors knowledge and by keeping only survey papers and papers from top-ranked venues (listing these venues of course). Moreover, authors should motivate why they decided not to opt on a structured survey methodology that are considered best practices by the research community. In this way, the reader would be more confident about the completeness of the survey results, and on the fact that results are trustworthy and not biased.}

Thank you for your positive feedback and for sharing your constructive suggestions. We are glad that our response addressed your initial concerns. 
Following your recommendation, we have revised the paper to include the description of the informal methodology we adopted for assembling relevant work.


We have added the corresponding illustration in Section \ref{sec_introduction} highlighted in blue color.\\

\subsection{Response to Reviewer \#2}

We would like to express our sincere gratitude for the reviewer’s insightful and detailed feedback. 
Your comments have been invaluable in improving the quality of our manuscript.
We have made substantial revisions to our manuscript and provided necessary clarifications on the points raised.
To better highlight our modifications, \add{all newly added content is emphasized in blue,} and \sout{the modified parts are marked with strikethrough.} \\


\review{\textbf{Review:} This new version of the paper includes some extended sections and new material, has changed the title and tried to answer the previous concerns of the reviewers, including the ones pointed out in my previous review. I believe both the original paper and this revised version were suitable works for the workshop at FSE, with a potential of engaging fruitful and interesting discussions. I am doubtful, however, about the relevance of the paper as a submission for TOSEM. While review and vision papers are welcome, I find this paper to be too broad in scope, implying that it is very hard to find a coherent longer term vision, as well as actionable insights. There are contradictory lines in the revision of the paper, that reflect this problem. On one hand, the authors have decided to change the title to concentrate in testing rather than quality assurance, but at the same time the scope is broadened in the paper, rather than make it more focused. As a consequence, the title promises something that is not present in the paper: the main aspect is indeed testing, but without depth since other aspects are also discussed.
}

Thank you for your thoughtful and detailed feedback. After careful consideration and discussions within our team, we have decided to focus the paper explicitly on software testing, as we believe this provides a clearer and more impactful scope for our work. 

To address your concerns about coherence and depth, we have made several substantial revisions to the manuscript. Specifically, we removed sections that were less closely related to software testing, such as subsection ``Continuous Integration and Modern Code Review'' (in
Section 2) and subsection ``AI Model Supply Chain and Security'' ``Software Development Process in AI Model-centric Paradigm'' (in Section 5). These changes were made to reduce the breadth of the paper and ensure the focus remains tightly aligned with testing.

Additionally, we have enhanced and refined the sections directly related to testing, adding more depth and actionable insights to strengthen the discussion. We believe these changes address the issue of the paper appearing overly broad and better align its content with the revised title. 

We greatly appreciate your constructive feedback, which has been instrumental in improving the clarity and focus of our work. We hope these revisions make the paper more suitable and relevant for TOSEM.\\


\review{\textbf{Review:} I do not agree with the new title in the open-source direction that it now has. Personally, I understand that open-source software refers to the software that is distributed together with the sources, typically with a strong emphasis in licensing terms that prevent future developers from “closing” the software, i.e., to just distribute it through binaries. For me, there is nothing in the paper that discusses particularly the open source culture, so the title has evolved in the wrong direction.}

Thank you for your valuable feedback. 
We understand your concerns regarding the emphasis on ``open-source'' in the title. 
Upon reflection, we agree that ``open-source'' may unintentionally shift the focus towards software distributed with source code and its licensing implications, which is not the primary emphasis of our paper.

To better align with the core discussion, we have reverted to using ``open-collaborative'' in the title. This term better captures our focus on the collaborative development practices enabled by the internet, highlighting the evolving paradigm of software testing in open environments, rather than specifically emphasizing source code availability. 
We believe this adjustment better reflects the paper's content and goals, and we appreciate your insight in helping us refine this aspect.\\


\review{\textbf{Review:} The challenges and opportunities is, in my opinion, the weakest part of this paper. Moreover, I believe that the problem is indeed in the so broad focus that the paper aims at. While I appreciate some of the new sections (e.g., 5.5. and 5.6), the paper ends up presenting just a list of very brief comments on what might be short term problems to tackle, without sufficient depth or concrete actionable insights. Overall, this is the feeling that I have with the paper, little insight on the situation regarding quality assurance in the AI era due to aiming at a very broad scope.
My recommendation for a TOSEM submission would be to concentrate on some specific topic and gain depth in it, and perhaps make some side comments on other complementary aspects.}


Thank you for your detailed feedback and for highlighting areas where the paper can be further improved. 
We understand your concerns regarding the challenges and opportunities section and the perception of a broad focus in the paper.

In this revised version, we have significantly narrowed the scope to focus specifically on software testing in the context of AI and open-collaborative development paradigms. 
This shift is reflected in both the title and the content of the paper. 
To enhance depth and provide actionable insights, we have made several changes: 

Refocusing the challenges and opportunities section: We have revised this section to concentrate on testing-related challenges, such as testing LLM-centric applications, testing and quality assurance for auto-generated code, and collaborative testing between human and AI. Each challenge is discussed in greater detail, some with examples and actionable recommendations for tackling them.

Removing less relevant content: Sections that were less directly related to software testing, such as subsection ``Continuous Integration and Modern Code Review'' (in
Section 2) and subsection ``AI Model Supply Chain and Security'' ``Software Development Process in AI Model-centric Paradigm'' (in Section 5), have been removed to avoid diluting the paper's focus.

Adding depth: We have expanded the discussions in key areas, such as leveraging LLMs to enhance testing, testing for LLMs and LLM-centric applications, and incorporating practical references to combining LLMs with traditional technologies. 
We have also addressed the testing challenges posed by LLM-as-agent systems like GUI agents, as well as non-functional concerns related to auto-generated code, to ensure the paper offers in-depth insights rather than brief overviews.

We appreciate your suggestion to focus on a specific topic, and this feedback has guided our revisions. 
By concentrating on testing, we aim to strike a balance between depth and breadth while retaining a broader perspective as complementary context.
We hope these revisions address your concerns and improve the clarity, depth, and relevance of the paper. Thank you again for your valuable input, which has been instrumental in guiding these improvements.\\


\review{\textbf{Review:} Throughout the paper: Artificial Intelligence (AI). Just indicate the abbreviation in the first occurence, then use AI. \\
Please revise subsection 3.3. It’s difficult to read, I believe there are some missing connectives. \\
When you say “System-Level”, it seems there is a missing noun. E.g., section 5.3. Please rephrase. \\
pp 4 The later ones -> The latter ones \\
pp 5 Once a issue -> Once an issue \\ 
pp 5 also short for crowdtesting -> also typically abbreviated as crowdtesting \\
pp5 during when -> during which \\
pp6 good first issue (GFIs) -> good first issues (GFIs) \\
pp6 there are studies to incorporate -> there are studies that analyze incorporating \\
pp7 “i.e., APIs.” It gives the feeling that APIs are deprecated libraries, which are not. Please rephrase. \\
pp7, section 4.2. Some sentences are too long and difficult to read. Please rephrase. \\
pp7 these information -> this information \\
pp8 to LLM to elicit -> to an LLM to elicit \\
pp8 GUI operation -> GUI operations \\
pp8 feedback to LLM -> feedback to the LLM \\
pp8 information to LLM -> information to the LLM \\
pp15 Collaborative between -> Collaborative interaction between.}

\textbf{Response:}  We apologize for these typos. 
As suggested, all of them have been fixed in the latest revision.  
We also rephrase sentences in Section 4.2 to make it more clear. \\
